Automatic Generation of Chatbots for Conversational Web Browsing

In this paper, we describe the foundations for generating a chatbot out of a website equipped with simple, bot-specific HTML annotations. The approach is part of what we call conversational web browsing, i.e., a dialog-based, natural language interaction with websites. The goal is to enable users to use content and functionality accessible through rendered UIs by "talking to websites" instead of by operating the graphical UI using keyboard and mouse. The chatbot mediates between the user and the website, operates its graphical UI on behalf of the user, and informs the user about the state of interaction. We describe the conceptual vocabulary and annotation format, the supporting conversational middleware and techniques, and the implementation of a demo able to deliver conversational web browsing experiences through Amazon Alexa.

==> approach.tex <==
\section{Conversational Web Browsing: Approach}
\label{sec:browsing}

The approach we explore in this paper is based on three main ingredients (i) purposefully designed bot \textit{annotations}, (ii) a \textit{middleware} comprised of chatbot generation and run-time units, and iii) a medium-specific \textit{conversational interface}. These components interact with each other as illustrated in Figure \ref{fig:architecture}.

Web developers enable conversational access by annotating their websites with bot-specific annotations. These annotations associate knowledge about how to generate a conversational agent (conversational knowledge) with specific HTML constructs. 
%
Initiating a conversational browsing session with a website equipped with these annotations then triggers the chatbot generation process. The \textbf{generation process} is about generating an application-specific bot tailored to the intents and vocabulary of the target website, while reusing as library of pre-canned, generic element-specific bots.
%
Using a conversational interface, in one of the supported mediums (e.g., telegram, Amazon Echo) the user can start a dialog with the website. At \textbf{run-time}, the bot processes the user requests in natural language and executes the appropriate actions on the browser on behalf of the user.

Supporting conversational browsing is neither technically nor conceptually trivial and requires weighing several options. The most important design decisions that resulted in the solution proposed in this paper are (see Figure \ref{fig:architecture} for an illustration of how the choices impact the implemented system architecture):
\begin{itemize}

\item \textbf{Domain vs. interaction knowledge}: Using a website generally requires the user to master two types of knowledge, \textit{domain knowledge} (to understand content and functionalities) and \textit{interaction knowledge} (to use and operate the site). It emerged during prototyping that this distinction is powerful to separate concerns in conversational browsing. Domain knowledge, e.g., about the research project and scientific publications, must be provided by the developer, as this varies from site to site and cannot be guessed automatically. Interaction knowledge, e.g., how to fill a form or read text paragraph by paragraph, can be pre-canned and reused across multiple sites. We thus distinguish between an \textit{application-specific} bot and a set of \textit{element-specific} bots [R1,R2]. The former masters the domain, the latter enable the user to interact with specific content elements like lists, text, tables, forms, etc.

\begin{figure}[t!]
\centering
  \includegraphics[width=1\columnwidth]{img/architecture.pdf}
  \caption{Functional architecture of conversational browsing infrastructure.}
  \label{fig:architecture}
\end{figure}

\item \textbf{Modularization}: Incidentally, the distinction between application- and ele\-ment-specific bots represents an excellent opportunity for modularization and reuse. Application-specific bots must be generated for each site anew; element-specific bots can be implemented and \textit{trained once and reused multiple times}. They can be implemented for specific HTML elements, such as a form, or they can be implemented for a very specific version thereof, e.g., a login form. There is no restriction for the development of pre-canned, element-specific bots. However, the presence of application- and element-specific bots introduces the need for a suitable bot selection logic.

\item \textbf{Bot selection}: As a user may provide as input any possible utterance at any instant of time, referring to either application-specific or element-specific intents, it is not possible to pre-define conversational paths through a website. Instead, some form of random access must be supported. We introduce for this purpose a so-called \textsf{bot manager}, which takes as input the utterance from the user and forwards it to the bots registered in the system [R5]. Depending on the context of the conversation (e.g., the last used bot) and the confidence provided by each invoked bot, it then decides which bot is most likely to provide the correct answer [R1,R2]. That answer is forwarded to the user. Thanks to the \textsf{bot manager}, the ensemble of application-specific and element-specific bots presents itself as one single bot to the user.

\item \textbf{Emulating user interactions}: Finally, once an intent is identified, a respective action may be performed. As the purpose of the bots is mediating between the user and the website, the actions must be able to communicate with the real site and mimic user interactions. While for simple, static sites parsing the HTML and generating HTTP Get requests might be enough, modern sites that also use client-side JavaScript ask for the use of a \textsf{headless browser} able to instantiate the DOM of a page, to apply CSS style sheets, to run JavaScript, and to provide programmatic access to it [R4]. Typical actions that can be supported are, for example, clicking a button, navigating to another page, or filling a form field.

\end{itemize}
